LazyPIM: Efficient Support for Cache Coherence in Processing-in-Memory Architectures

Processing-in-memory (PIM) architectures have seen an increase in popularity recently, as the high internal bandwidth available within 3D-stacked memory provides greater incentive to move some computation into the logic layer of the memory. To maintain program correctness, the portions of a program that are executed in memory must remain coherent with the portions of the program that continue to execute within the processor. Unfortunately, PIM architectures cannot use traditional approaches to cache coherence due to the high off-chip traffic consumed by coherence messages, which, as we illustrate in this work, can undo the benefits of PIM execution for many data-intensive applications. We propose LazyPIM, a new hardware cache coherence mechanism designed specifically for PIM. Prior approaches for coherence in PIM are ill-suited to applications that share a large amount of data between the processor and the PIM logic. LazyPIM uses a combination of speculative cache coherence and compressed coherence signatures to greatly reduce the overhead of keeping PIM coherent with the processor, even when a large amount of sharing exists.We find that LazyPIM improves average performance across a range of data-intensive PIM applications by 19.6%, reduces off-chip traffic by 30.9%, and reduces energy consumption by 18.0%, over the best prior approaches to PIM coherence.

==> sections/evaluation2.tex <==
% !TEX root=../paper.tex

\section{Evaluation}
\label{sec:eval}

We examine how LazyPIM compares with prior coherence
mechanisms for PIM.
Unless otherwise stated, we assume that LazyPIM employs partial kernel commits
as described in Section~\ref{sec:arch:partial}, and that it uses PIM-DBI, where
all dirty data in the processor caches is written back every 800K processor cycles.
We show results normalized to a processor-only baseline (\emph{CPU-only}),
%\footnote{\label{foot:motiv}See
%Sec.~\ref{sec:motivation} for the definition.}
and compare to PIM execution using fine-grained coherence (\emph{FG}), coarse-grained locks 
(\emph{CG}), or non-cacheable PIM data (\emph{NC}),
as described in Section~\ref{sec:motivation:naive}.

We first analyze the performance improvement of LazyPIM in
Section~\ref{sec:eval:perf}.
We then analyze the off-chip traffic reduction (Section~\ref{sec:eval:offchip})
and energy savings (Section~\ref{sec:eval:energy}) of LazyPIM.
Finally, we study the effects of partial kernel commits (Section~\ref{sec:eval:partial}), 
signature size (Section~\ref{sec:eval:signature}), and PIM-DBI
(Section~\ref{sec:eval:pimdbi}) on the performance of LazyPIM.



%\vspace{-3pt} %tcolorbox hack
\subsection{Performance}
\label{sec:eval:perf}

%Fig.~\ref{fig:performance} (left) shows the performance, normalized to FG, of PageRank using Gnutella
%as we increase the thread count.  LazyPIM improves performance by up to 72\% 
%over NC, 3.5x over CG, and 88.3\% over FG.
%With NC, the processor threads incur a large
%penalty from going to DRAM frequently.  CG 
%suffers greatly due to (1)~flushing dirty cache lines, and (2)~blocking all processor threads that access PIM
%data during execution (see Sec.~\ref{sec:motivation}). In fact, processor threads are blocked for up to
%73\% of execution time with CG.  With more threads, the effects of blocking worsen CG's performance.

%\begin{tcolorbox}
Figure~\ref{fig:performance2} shows the performance improvement for a 16-core 
architecture (with 16 processor cores and 16~PIM cores) across all of our 
applications and input sets.
% for 16 threads.
Without any coherence overhead, the ideal PIM mechanism (Ideal-PIM, as defined in Section~\ref{sec:motivation:naive}) 
significantly outperforms CPU-only across all applications, showing the potential of PIM execution on these workloads.
    % Ideal-PIM performs significantly better compared to CPU-only baseline across all applications. 
% As shown in Fig.~\ref{fig:performance} (right),
The poor handling of coherence by CG and NC, and by FG in a number of cases, leads to drastic performance losses compared to Ideal-PIM,
indicating that an efficient coherence mechanism is essential for PIM performance.
For example, in many cases, NC and CG actually perform \emph{worse} than CPU-only, and for
PageRank running on the Gnutella graph, all prior mechanisms degrade performance.  
In contrast, LazyPIM consistently retains most of Ideal-PIM's benefits for all applications, coming within
11.4\% of the Ideal-PIM performance, on average. 
 LazyPIM outperforms all other approaches, improving average performance by 18.3\% over FG, 40.4\%
 over CG, 66.7\% over NC, and 33.5\% over CPU-only. 
%even though 38.5\% of its kernels roll back due to concurrent accesses from the processor.


\begin{figure}[h]
    \centering
    \vspace{-5pt}
    \includegraphics[width=\linewidth]{figures/Speedup16.pdf}%
    \vspace{-8pt}%
    \caption{Speedup for all applications with 16~threads, normalized to CPU-only execution.}
    \label{fig:performance2}
    \vspace{-5pt}
\end{figure}


We select PageRank using the ArXiv input set for a case study on how
performance scales as we increase the core count, shown in 
Figure~\ref{fig:performance1}.
 Ideal-PIM significantly outperforms CPU-only at all core counts. 
With NC, the processor threads
 incur a large penalty for going to DRAM frequently to access the PIM data region.
 CG suffers greatly due to (1)~flushing dirty cache lines, and (2)~blocking all processor
 threads that access PIM data during execution. In fact, processor threads 
 are blocked for up to 73.1\% of the total execution time with CG. With more core, the effects of 
 blocking worsen CG's performance. FG also loses a significant portion of Ideal-PIM's 
 improvements, as it sends a large amount of off-chip messages.
Note that FG, despite its high off-chip traffic, scales better with core count 
than CG and NC, as it neither blocks processor cores nor slows down CPU execution.
LazyPIM improves performance at all core counts.
%, as it retrieves 
%the data directly from DRAM and doesn't generate any off-chip coherence traffic.}
%The reason is NC doesn't block
%processor cores. It also doesn't slow down PIM execution, as it retrieves 
%the data directly from DRAM and doesn't generate any off-chip coherence traffic.}
% to the main coherence directory. }
%\end{tcolorbox}

% Figure 3 shows execution time for PageRank algorithm in Ligra using Gnutella peer-to-peer network graph as input for different number of PIM-threads. As it is shown in the figure, LazyPIM reduces execution time up to 2x compared to non-cacheable and up to 6.5x compared to coarse-grained baseline. Coarse-grained baseline has huge performance penalty because before any PIM thread start executing the kernel, all caches need to be scanned to flush-back the dirty PIM data. Furthermore, during PIM execution, all CPU threads that access PIM data are blocked until PIM is done. Our result show that on average, up to Kx of CPU memory accesses, including PIM and non PIM-data, are blocked during kernel execution. Non-cacheable also hurts CPU threads/system performance since it forces all access from CPU to go to DRAM.


\begin{figure}[t]
    % \vspace{-3pt}
%\begin{tcolorbox}
    \centering
        \centering
        \includegraphics[width=\linewidth]{figures/Speedup4.pdf}%
\vspace{-10pt}%
    \caption{Speedup vs.\ thread count for PageRank with arXiV graph, normalized to CPU-only execution.}
    \label{fig:performance1}
%    \vspace{-11pt}
%\end{tcolorbox}
   \vspace{-12pt}
\end{figure}


 %Note that we conservatively assumed that the bloom filter always have 20\%
% false positive rate, which leads to 0.49\% increase in the total execution time.}
%\end{tcolorbox}

%Fig.~\ref{fig:performance} (right) shows the performance improvement across all 
%of our applications and input sets for 16~threads.  
%LazyPIM improves average performance over the next best approach (FG) by 
%17.6\%.  
%LazyPIM outperforms all of the other approaches, even though 30.1\% of its 
%kernels roll back due to concurrent accesses from the processor.  
%For our graph applications, LazyPIM improves performance at \emph{all} thread 
%counts.



%, as
%off-chip PIM traffic is only a small part of the total traffic 
%(Sec.~\ref{sec:eval:offchip}).  
%For DBx1000, LazyPIM's performance is nearly identical to CG and NC.
%The PIM data region in DBx1000 (the B-tree index) is
%much smaller than in our graph workloads, and as a result, a much smaller 
%number of requests access the index.  The \emph{percentage} of sharing by
%the processor remains
%high (Sec.~\ref{sec:motivation}), so even with fewer requests, many
%kernel rollbacks occur (e.g.,
%54\% of kernels for 16~threads).  As the kernel execution time is short, most
%rollbacks are not due to concurrent accesses, but are the result of dirty 
%processor cache lines.  We can significantly reduce the probability of conflicts by 
%using the Dirty-Block Index~\cite{seshadri2014dirty} to track dirty PIM data 
%and invoke periodic writebacks in the background.  Our preliminary analysis shows that 
%even if we eliminate only 25\% of the rollbacks, LazyPIM can \emph{improve}
%DBx1000 performance over CG and NC by 5\%.


% For DBx1000, though LazyPIM reduces PIM data traffic by 24\%, its
% performance is nearly identical to NC and CG.
% We find two reasons for this.  First, the PIM kernel selected for
% DBx1000 (the indexing operation) is very short (at least 12x shorter
% execution time than in our graph applications).  Second, as we mentioned before, 
% the PIM data (the B-tree index) accounts for a much smaller portion of the total application data than 
% our graph applications, which in turn significantly reduces the sharing that
% occurs between PIM kernels and processor threads.  As a result, any benefits
% of LazyPIM from the bandwidth savings are offset by the fact that many kernels
% in DBx1000 need to roll back (e.g., 54\% of kernels for 16~threads).
% 
% Looking further, we find that most of these rollbacks are due to dirty cache
% lines, which can be mitigated by adding a Dirty-Block
% Index (DBI)~\cite{seshadri2014dirty}.
% If we use DBI to track PIM data in the CPU caches, and invoke PIM data
% writebacks in the background (i.e., when PIM kernels are not executing), we
% significantly reduce the probability of conflicts.  Our preliminary analysis 
% shows that if we eliminate only 25\% of the rollbacks, LazyPIM can \emph{improve}
% performance over NC and CG by 5\%.

%Figure 4 shows performance result across variety of applications in Ligra and DBx1000. LazyPIM improves performance in almost all applications. For DBx1000, although LazyPIM improves bandwidth by Kx, the performance is almost the same compared to Non-cacheable and Coarse-grained locking baseline. There are a couple of reasons for that. First, PIM kernel in dbx1000, which perform indexing operation, is small and short-running (at least 12X smaller than Ligra kernels in terms of execution time), and more importantly, PIM-data in DBx1000 (B-tree index) account for significantly smaller portion of total application data than PIM-data in Ligra (Graph), which in turns leads to smaller sharing between PIM threads and CPU threads. As a result, since off-chip traffic is not as high as Ligra, rollbacks of PIM threads, which happen in on average 54 of total kernels, has significant affect on performance. After further analysis, we realized that almost all of the conflicts/rollback in DBx1000 are due to dirty cache lines. This can be alleviated using ideas such as DBI. We can employ DBI for only PIM-data in CPU caches and aggressively write-back PIM dirty cache lines on background. That could significantly reduce the conflict in dbx1000. Our analysis shows that even 25 reduction in those conflicts lead to 10 performance improvement compared to Non-cacheable and Coarse-grained lock.

We conclude that LazyPIM successfully harnesses the benefits of
speculative coherence updates to provide performance improvements in a wide
range of PIM execution scenarios, when prior coherence mechanisms cannot
improve performance and often degrade it.


\subsection{Off-Chip Traffic}
\label{sec:eval:offchip}

Figure~\ref{fig:traffic2} shows the normalized off-chip traffic of the PIM 
coherence mechanisms for our 16-core system.  LazyPIM significantly 
reduces \emph{overall} off-chip traffic, with an average reduction of 31.1\% 
over CG, the best prior approach in terms of traffic.
% NC, the best prior approach.}
CG has greater traffic than LazyPIM mainly because CG
has to flush dirty cache lines before each PIM kernel invocation,
while LazyPIM takes advantage of speculation to perform \emph{only} the
\emph{necessary} flushes \emph{after} the PIM kernel finishes execution.
As a result, LazyPIM reduces the flush count (e.g., by 92.2\% for
Radii using arXiV), and thus lowers overall 
off-chip traffic (by 48.1\% for our example).
NC's traffic suffers from the fact that \emph{all} processor accesses to the
PIM data region must go to DRAM.
With respect to CPU-only, LazyPIM provides an average traffic reduction of 
71.1\%.


\begin{figure}[h]
    \vspace{-7pt}
%\begin{tcolorbox}
    \centering
    \includegraphics[width=\linewidth]{figures/Traffic16.pdf}%
    \vspace{-8pt}%
    \caption{16-thread off-chip traffic, normalized to CPU-only execution. \emph{Note that lower is better.}}
    \label{fig:traffic2}
   % \vspace{-2.5pt}
%\end{tcolorbox}
\vspace{-5pt}
\end{figure}


Figure~\ref{fig:traffic1} shows the normalized off-chip traffic as the 
number of cores increases, for PageRank using the arXiV graph.  
% (up to 97.2\% over CPU-only, 81.9\% over FG, 72.3\% over CG, and 92.9\% over NC), 
LazyPIM's traffic scales better with core count than prior PIM 
coherence mechanisms.
%than the other mechanisms. 
Due to false sharing, the number of flushes for CG scales \emph{superlinearly} with 
thread count (not shown), increasing 13.1x from 4 to 16~threads.
%As shown in Sec.~\ref{sec:motivation}, processor accesses represent a large
%fraction of the total number of accesses to PIM data.
NC also scales poorly with core count, as more processor threads generate a greater number of accesses.  In
contrast, LazyPIM allows processor cores to cache PIM data, by enabling
coherence efficiently, which lowers off-chip traffic on average by 85.9\% with respect
to NC.

\begin{figure}[h]
    \vspace{-7pt}
    \centering
    \includegraphics[width=\linewidth]{figures/Traffic4.pdf}%
    \vspace{-8pt}%
    \caption{PageRank off-chip traffic sensitivity to thread count with arXiV graph, normalized to CPU-only execution. \emph{Note that lower is better.}}
    \label{fig:traffic1}
   \vspace{-5pt}
\end{figure}


% As
% we discussed in Sec.~\ref{sec:motivation}, pointer-chasing workloads such as
% PageRank have access patterns that are difficult to predict, thus it is not
% feasible to flush back only the dirty lines used by the PIM kernel, even though
% this is a small portion of the total number of dirty cache lines.  
%At this point, we know \emph{exactly} which lines were
%touched (if any), which % this is only for FB 16 thread page rank

% The majority of traffic for Coarse-grained baseline is because of all dirty cache lines that need to be flushed back before PIM threads start execution. Since PIM threads needs to perform pointer-chasing to traverse the graph, and there is no way to predict the which path will be taken, it is required to flush back almost all dirty PIM cache lines which hold graph data, even though PIM thread does not touch those data during graph traversal. As the number of threads increases, the number of dirty cache lines as well false sharing becomes significantly higher, and thus, the off-chip traffic increases by Kx from 4 threads to 16 threads. We expect that this traffic will drastically increase when thread numbers scales to 32 or 128. In LazyPIM, however, PIM-thread goes over Kernel speculatively, and as a result, flush-backs only those cache-lines that cause conflict. This significantly reduces the amount of flush back (on average by Kx), and therefore, off-chip traffic.  


%and greatly lowers off-chip traffic 
%generated by the processor.


% Non-cacheable baseline suffers from the fact that all CPU accesses to PIM data need to go off-chip, leading to substantial off-chip traffic. As we mentioned in motivation section, this accesses from CPU accounts for large fraction (up to 36\% for Ligra applications and 35\% for dbx1000) of accesses to PIM data. As it is presented in Figure1, Non-cacheable off-chip traffic increases dramatically when thread number scales to 16. LazyPIM, in contrast, allows CPU threads to benefit from caching PIM data while lowering the off-chip traffic significantly.

% In figure 2 we present off-chip traffic for LazyPIM in comparison with Coarse-grained baseline and Non-cacheable baseline, for various applications in Ligra framework as well as dbx1000. The workload for Ligra is peer-to-peer network and number of PIM threads are 16. As it is illustrated in Figure 2, LazyPIM significantly reduce off-chip traffic across different applications

%Unlike with the graph applications, there is only a small improvement in
%off-chip traffic when LazyPIM is used for DBx1000 (7\% better than NC, and 2\%
%better than FG).  Looking closer, we actually
%find that LazyPIM \emph{does} significantly reduce the off-chip \emph{PIM} traffic,
%by 62\% over NC and by 24\% over FG.  However, the selected PIM
%kernel, indexing, is very short (at least 12x shorter in 
%execution time than our graph application kernels).
%As a result, the \emph{total}
%off-chip traffic is dominated by accesses to \emph{non-PIM} data (which account for
%90\% of the total traffic).  Hence, the overall improvement is low.

We conclude that the efficient approach to coherence employed by LazyPIM allows
it to successfully provide fine-grained coherence behavior while still 
delivering reductions in off-chip traffic.


\subsection{Energy}
\label{sec:eval:energy}

Figure~\ref{fig:energy} shows the energy consumption of the PIM coherence 
approaches for our 16-core system, normalized to CPU-only, across all of
our applications and input sets.  We find that LazyPIM significantly reduces
energy consumption, by an average of of 43.8\% over FG, 18.9\% over CG,
65.0\% over NC, and 18.5\% over CPU-only.  The main energy improvement for
LazyPIM over CPU-only comes from a reduction in interconnect and memory
utilization, as LazyPIM successfully reduces data movement across the off-chip
channel.


\begin{figure}[h]
    \centering
    \vspace{-5pt}
    \includegraphics[width=\linewidth]{figures/Energy.pdf}%
    \vspace{-8pt}%
   % \caption{Speedup sensitivity to thread count for PageRank with Facebook graph (left), and speedup for all applications with 16~threads (right) for coherence mechanisms, normalized to CPU-only.}
    \caption{Energy for all applications with 16~threads normalized to CPU-only execution.}
    \label{fig:energy}
    \vspace{-5pt}
\end{figure}


Other PIM coherence approaches are unable to retain these benefits, as FG, CG, 
and NC all consume more energy due to their poor handling of coherence.
CG has a large number of writebacks, which leads to increased L1 and L2 cache
lookups and a large amount of traffic sending dirty data back to DRAM 
preemptively.  Thanks to these writebacks, the energy consumption of the HMC
memory alone increases by 18.9\% on average over CPU-only, canceling out CG's
net savings in interconnect energy (which was reduced by 49.1\% over CPU-only).
The energy consumption of NC suffers greatly from the large number of memory
operations that are redirected from the processor caches to DRAM.  While the 
cache energy consumption falls by only 7.1\%, interconnect and HMC energy
increase under NC by 3.1x and 4.5x, respectively.
For FG, the large number of coherence messages transmitted between the 
processor and the PIM cores undoes the energy benefits of moving computation
to DRAM.

We conclude that the speculative coherence update approach used by LazyPIM is
effective at retaining the energy benefits of PIM execution.

% Fig.~\ref{fig:energy} shows the normalized energy of the PIM coherence mechanism for a 16-core
%  architecture across all of our applications and input sets (It is assumed that CPU-only is equipped with HMC).
%  LazyPIM significantly reduces energy by 42.7\% over FG, 18.0\% over CG. 68.1\% over NC and 16.5\% 
% over CPU-only baseline. The main energy improvement come from reduction in interconnect and HMC energy, as LazyPIM
%  significantly reduces the data movement over the off-chip channel and lower the accesses to DRAM.  Poor
%  handling of coherence by FG, CG, and NC eliminate almost all of the PIM energy improvement over CPU-only. 
% With CG, large number of write backs leads to significant number of lookups to L1 and L2 caches as well as large amount of traffic
%  over off-chip channel to HMC. Because of the additional look ups and write-backs, CG loses all of the CPU cache energy saving PIM 
%  provides, slightly increasing cache energy on average by 0.2\% over CPU-only. CG also increases HMC energy on average by 18.9\% 
%  over CPU-only due to extra writebacks to HMC. Note that CG still reduces interconnect energy by 49.1\% 
%  over CPU-only by eliminating a significant portion of data movement. 
% . NC suffers greatly from large number of accesses from CPU to PIM data, 
% increasing interconnect and HMC energy over CPU-only by 3.1X and 4.5X respectively. NC reduces
% cache energy by 7.1\% over CPU-only by replacing majority of CPU L1 and LLC accesses with HMC and PIM cache
% accesses. FG generates a large number of coherence messages over off-chip channel as well as many write-backs
% to HMC as a result of fine-grained coherence between PIM cores and
%  CPU cores, which result in on average 2.3X increase in HMC energy. Similar to NC, FG reduces cache energy by 4.1\% over CPU-only. 
% It also decreases interconnect energy by 47.8\% over CPU-only. 


\subsection{Effect of Partial Kernel Commits}
\label{sec:eval:partial}

As we discussed in Section~\ref{sec:mech:partial}, dividing a PIM kernel into
smaller partial kernels allows LazyPIM to lower both the probability of 
coherence conflicts and false positives.  Figure~\ref{fig:conflictrate} shows
the extent of the benefits that partial commits offer, for a signature size of
2~Kbits, for two representative 16-thread workloads: Components
using the Enron input set, and HTAP-128  
If we study an idealized version of full kernel commit, where no false 
positives exist, we find that a relatively high percentage of commits contain
conflicts (47.1\% for Components and 21.3\% for HTAP).  Using realistic
signatures for full kernel commit, which includes the impact of false 
positives, the conflict rate increases to 67.8\% for Components and 37.8\% for
HTAP.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/conflictrate.pdf}
    \vspace{-5pt}%
   % \caption{Speedup sensitivity to thread count for PageRank with Facebook graph (left), and speedup for all applications with 16~threads (right) for coherence mechanisms, normalized to CPU-only.}
    \caption{Effect of full kernel commits vs.\ partial kernel commits on conflict rate of representative 16-thread workloads.}
    \label{fig:conflictrate}
    \vspace{-9pt}
\end{figure}


Whenever a conflict is detected, a rollback must be initiated.  In the case of 
the full kernel signatures above, this means that approximately half of all
commit attempts force LazyPIM to roll back to the beginning of the entire
kernel.  As Figure~\ref{fig:conflictrate} shows, our partial kernel commit
technique significantly reduces this burden.  Even factoring in false 
positives, the conflict rate drops to 23.2\% for Components and 9.0\% for
HTAP.  Further helping partial kernel commit is the fact that in the cases
when rollbacks do occur, the length of the rollback is smaller, as only a
small portion of the kernel must be re-executed.

We conclude that partial kernel commit is an effective technique at keeping
the overheads of LazyPIM rollback low.

% As we discussed in section 4.2, committing large kernels could increase the chance of conflicts and false positive rate
%  as it could exceed the signature capacity. Dividing the PIM kernel into smaller chunks enables LazyPIM
%  to lower the chance of conflict and false positive rate. Fig.~\ref{fig:conflictrate} illustrates the effect of partial commit on conflict
%  rate for 16 threads Components using email-Enron graph and 16 threads IMDB using 32K transactional and 128 analytical queries, compared to committing a full kernel.
%  Assuming 2Kb ideal signatures with no false positive rate, committing full kernel (no partial commit)
%  leads to a relatively high number of conflicts (47.1\% for Components and 21.3\% for HTAP).
%  Replacing ideal signature with real
%  signature increases conflict rate to 67.8\% for Components and 37.8\% for IMDB, due to presence of false positive. With
%  partial commit (every 250 memory addresses and 1M committed instructions), conflict rate drops to 23.2\% for Components (65.7\% reduction)
%  and 9.0\% for IMDB..

% The effectiveness of partial commit mainly relies on the size of each chunk. Size of each chunk
%  is determined based on both number of memory accesses and number of committed instructions. The former plays a
%  significant role in effectiveness of partial commit, as it keep false positive rate low and lower the chance of 
% conflicts. The latter, as we mentioned before, is assumed to be 1M to prevent low memory footprint kernels to
%  execute many instruction before reaching the memory limit. Here we evaluate the effect of chunk size, based
%  on number of memory accesses. Fig.~\ref{fig:partialset} shows the normalized latency, traffic and conflict rate for 16 threads Components
%  using email-Enron graph and 16 threads IMDB using 32K transactional and 128 analytical queries across
%  different chunk size. As it is shown, having smaller chunk size leads to lower conflict
%  rate and false positive rate, and thus, lower latency. Decreasing chunk size from 350 to 150 reduces
%  conflict rate and latency by 25.5\% and 5.4\% for Components and 49.2\% and 25.5\%. On the other hand, smaller chunk size means
%  more partial commit need to be done, and as a result, more signatures need to be transferred over the off-chip
%  channel. Therefore, as it is shown in Fig.~\ref{fig:partialset}, lowering the signature size from 350 to 150 increases traffic by 34.5\% and 18.3\%, 
 % for IMDB and Components respectively..   
% 
% \begin{figure}[t]
%     \centering
%     \begin{minipage}{\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/partialset.pdf}
%     \end{minipage}%
%    % \caption{Speedup sensitivity to thread count for PageRank with Facebook graph (left), and speedup for all applications with 16~threads (right) for coherence mechanisms, normalized to CPU-only.}
%     \caption{Effect of partial commit size on latency, traffic and conflict rate for 16 threads Components using email-Enron graph and 16 threads IMDB using 32K transaction and 128 analytic queries, normalized to CPU-only.}
%     \label{fig:partialset}
% \end{figure}


\subsection{Effect of Signature Size}
\label{sec:eval:signature}

As we discussed in Section~\ref{sec:arch:signature}, the signature size has a
direct effect on the false positive rate during conflict detection.  Larger
signatures have lower false positive rates, which in turn reduce the number of
rollbacks due to conflicts.  However, larger signatures consume a greater 
amount of off-chip traffic, as we need to send both the \pimreadset and the
\pimwriteset every time a partial kernel completes.

We study the impact of signature size on three factors: execution time, 
off-chip traffic, and the conflict rate.  Note that for all signature sizes, we
continue to store 250~addresses per signature using partial kernel commit.  Figure~\ref{fig:sigsize}
shows these three factors, with execution time and off-chip traffic normalized
to CPU-only, for our two representative 16-thread workloads.  Increasing the signature size from 2~Kbits to 8~Kbits reduces the
conflict rate by 30.0\% for Components and by 29.3\% for HTAP, which in turn
results in a reduction in execution time of 10.1\% and 10.9\%, respectively,
as the lower conflict rate results in a smaller number of rollbacks.  The
reduction in conflict rate is a direct result of the lower false positive rate
with 8~Kbit signatures (a reduction of 31.4\% for Components and 40.5\% for
HTAP).  However, we see that this comes at the cost of increased off-chip 
traffic, as the 8~Kbit signature requires 32.7\% more traffic for Components
and 31.4\% more traffic for HTAP.

% In this section we evaluate the effect of signature size on latency, traffic and conflict rate. As we
%  discussed in section 5.4.2,  signature size has direct effect on the false positive
% rate. Large signature lowers the false positive rate and in turn, the conflict rate,
%  which has direct correlation with the execution time. Signature size also directly affects off-chip
%  traffic since PIMReadSet and PIMWriteSet are transmitted over the off-chip bus. 
% 
% Fig.~\ref{fig:sigsize} shows normalized latency, traffic and conflict rate for 16 threads
%  Components using email-Enron graph across three different signature sizes. Increasing
%  signature size from 2Kb to 8Kb leads to 30.0\% reduction in conflict rate, 
% and as a result of smaller number of rollbacks, result in 10.1\% reduction in
%  total execution time. This reduction in conflict rate is mainly because of less number
%  of false positive rate (31.4\% reduction). On the other hand, increasing signature size from 2Kb to
%  8Kb generates 32.7\% more off-chip traffic since a larger signature is transmitted over the
%  off-chip channel. Our result indicates that using a small 2Kb signature strikes a balance between latency and traffic across our workloads.


\begin{figure}[h]
    \vspace{-3pt}
    \centering
    \includegraphics[width=0.85\linewidth]{figures/sigsize.pdf}
    \vspace{-6pt}%
    \caption{Effect of signature size on representative 16-thread workloads, with execution time and off-chip traffic normalized to CPU-only execution.}
    \label{fig:sigsize}
    \vspace{-3pt}
\end{figure}


From our evaluations, we conclude that using a smaller 2~Kbit signature strikes
a good balance between execution time and off-chip traffic across all of our
workloads.


\subsection{Effect of PIM-DBI}
\label{sec:eval:pimdbi}

As we mentioned in Section~\ref{sec:arch:pimdbi}, LazyPIM can reduce the 
occurrence of dirty conflicts by periodically invoking PIM-DBI to write back 
the dirty data in the processor caches.  One key trade-off with PIM-DBI is how
often we trigger writebacks.  While a more frequent trigger can further reduce
the rate at which dirty conflicts occur, each trigger event consumes time and
off-chip bandwidth, and excessively frequent triggering can undo the savings
of avoiding dirty conflicts.

Figure~\ref{fig:dbi} shows the effect of invoking PIM-DBI at different rates,
compared to not invoking PIM-DBI at all (labeled \emph{No DBI} in the figure).
As we did in Section~\ref{sec:arch:signature}, we study the impact on execution 
time, off-chip traffic, and the conflict rate, with execution time and off-chip 
traffic normalized to CPU-only, for 16-thread Components and HTAP-128.
We explore three trigger frequencies: \emph{Slow}, \emph{Mid}, and 
\emph{Fast}, which trigger PIM-DBI every 800K, 500K, and 100K processor cycles,
respectively.  Using \emph{Fast} PIM-DBI triggering reduces the conflict rate 
by 38.9\% for Components and by 46.5\% for HTAP, mainly as a result of the
large drop (70.3\% for Components, 68.1\% for HTAP) in the number of dirty
cache lines belonging to the PIM data set when PIM kernels execute.
The use of PIM-DBI improves execution time, with \emph{Slow} triggering reducing
execution time by 9.3\% and 8.6\% for Components and HTAP, respectively, and
more aggressive \emph{Fast} triggering reducing execution time by 15.4\% and
17.3\%.  As we saw with signature size, more aggressive PIM-DBI triggering 
consumes greater off-chip bandwidth, with \emph{Slow} triggering generating
25.8\% more traffic for Components, and with \emph{Fast} generating 2.7x the
total traffic generated without PIM-DBI.

% In this section we analyze the effectiveness of PIM-DBI. As we mentioned in section 5.5, using PIM-DBI to invoke periodic
% PIM data write-backs, LazyPIM could lower the number of dirty PIM cache lines which leads to significant reduction in dirty conflicts and false positive rate. The important point is how frequent the periodic write-back is invoked. If it invokes very infrequent, it won’t be able to affect the conflict rate while if it happens too frequent, it generates a large amount of off-chip traffic. 


% Fig.~\ref{fig:dbi} shows effect of periodic write-backs with different frequency using PIM-DBI on latency, traffic and conflict rate for 16 threads Components using email-Enron graph normalized to CPU-only baseline. Zero means that no write-back happens. Low, Mid and High represent different frequency of write-backs using PIM-DBI (high is the most aggressive configuration).
%  As it is shown, conflict rate drops as we increase the frequency of write-backs. Using PIM-DBI with High frequency leads to 38.9\% decrease in conflict rate. This is mainly because of significant reduction (70.3\%) in the number of dirty PIM cache lines as we increase the frequency from Zero to High.
%  The reduction in conflict rate in turn has a direct effect on execution time. With smaller number of rollbacks, latency reduces by
%  15.4\% using High frequency PIM-DBI compares to Zero frequency. However, having High frequency DBI comes at a
%  cost of significant increase in traffic, as we aggressively write-back a large amount of PIM data. As it is shown
%  in Fig.~\ref{fig:dbi}, increasing PIM-DBI frequency leads to up 2.7X increase in total off-chip traffic. For example, 67.19\% of
%  total off-chip traffic comes from PIM-DBI when High frequency configuration is used. This result indicates a clear trade-off
%  between latency and traffic when PIM-DBI is employed. We used low frequency PIM-DBI as it strikes a balance between latency and traffic.


\begin{figure}[h]
    \vspace{-5pt}
    \centering
    \includegraphics[width=0.85\linewidth]{figures/dbi.pdf}
    \vspace{-6pt}%
    \caption{Effect of PIM-DBI trigger rate on representative 16-thread workloads, with execution time and off-chip traffic normalized to CPU-only execution.}
    \label{fig:dbi}
    \vspace{-5pt}
\end{figure}


We conclude that 
(1)~using PIM-DBI is good for performance, 
(2)~PIM-DBI triggering frequency exposes a tradeoff between execution time and
off-chip bandwidth, and
(3)~\emph{Slow} triggering frequency for PIM-DBI strikes a
good balance between dirty conflict reduction and off-chip traffic
utilization.


==> sections/optimization.tex <==
% !TEX root=../paper.tex

\section{Optimizations}
\label{sec:optimize}

In this section we discuss ...

\subsection{Dividing kernels}
\label{sec:optimie:divide}
PIM mainly benefits memory-intensive application, as they generate many memory accesses.
 Naturally, one can expect that there could be PIM kernels that generate a lot of reads
 and/or writes. Such large kernels could increase the false positive rate of the bloom
 filters, increase the number of conflicts, and even exceed the L1 or bloom filter
 capacity. Rolling back such kernel is also very expensive, as it wastes
 a massive amount of work done by PIM. We can simply avoid this by dividing the
 PIM kernel into smaller chunks, where we perform a commit
after each chunk completes. This lowers the number of speculative updates
 and the number of addresses that must be tracked by our signatures.
 It also lowers the chance of conflict as each chunk touches less addresses and
 commits the updates right after it completes. 

The benefit/effectiveness of this optimization mainly relies on the
 size of each chunk. If a chunk is too small, even though it significantly
 lowers the chance of conflicts as well as false positive rate of bloom filters,
 it generates large amount of traffic, as it needs to update the coherence state frequently,
 undoing most of the benefit of LazyPIM’s coarse-grained atomicity. On the other hand,
 if the chunk is not small enough, it cannot achieve the true benefit of this optimization. 


\subsection{Dirty cache lines}
\label{sec:optimize:dbi}



==> sections/rebuttal.tex <==
% !TEX root=../rebuttal.tex


\section*{{\Large AUTHORS' RESPONSE}}
\label{sec:rebuttal}

We thank the reviewers for their helpful feedback. We addressed all
comments from the reviewers. The following is
a list of the major changes we made to the paper (highlighted in yellow in the paper):

\vspace{10pt}

\begin{enumerate}
\setlength\itemsep{15pt}

\item 
In \textbf{Sections~3 and~6}, \changes{following Reviewer~3's recommendation,} we replaced DBx1000 with an in-house in-memory database (IMDB) that supports Hybrid Transactional/Analytical Processing (HTAP) workloads.  \changes{We found that the DBx1000 kernels were not a good fit for PIM execution. In place of DBx1000, we used a database workload that includes analytical queries, which have been shown by prior work to be a good fit for PIM.}  We found that LazyPIM outperforms all prior PIM coherence mechanisms when used for \changesII{the} IMDB.  \changes{\textbf{Section~5} was modified to include a description of the workload, and} \textbf{Figures~3 and~4} were updated to include this new workload.
\\\emph{This addresses Reviewer~3's comments.}


\item 
In \textbf{Section~3}, we improved our explanation of why data sharing is necessary and unavoidable when many important applications, such as graph workloads and databases, are adapted for PIM execution.
\\\emph{This addresses Reviewer~1's comments.}


\item 
In \textbf{Sections~3 and~6}, we updated our results to use a CPU-only baseline, where the entire application is run without using the PIM cores, to show that these workloads are indeed a good fit for PIM execution.  We also included results for a theoretical ideal PIM mechanism, where there is no latency or bandwidth cost for coherence requests, to show the potential these applications have without the overhead of coherence.  \changes{We replaced \textbf{Figure~1} for our motivation, to demonstrate how our kernels are a good fit for PIM, but that prior PIM coherence mechanisms cannot take advantage of \changesII{these PIM kernels} due to \changesII{the mechanism} overhead.  We also added these comparison points to \textbf{Figures~3 and~4}.}
% \textbf{Figures~1, 3, and~4} are all now normalized to the CPU-only performance.  
\\\emph{This addresses Reviewer~1's and Reviewer~3's comments.}


\item 
In \textbf{Section~4.1}, we added a short explanation of the potential data dependencies that we did not cover in the last submission, and how these these \changesII{potential dependencies do not lead to conflicts that affect our mechanism} due to our use of coarse-grained atomicity.
\\\emph{This addresses Reviewer~2's comments.}


\item
We significantly improved the accuracy of our results since our last submission (which included preliminary results for our work).  In particular, we now use a more realistic model within the full-system simulator for the coarse-grained lock (CG) and non-cacheable (NC) mechanisms.
%, ensuring that no coherence messages are exchanged for both of these mechanisms during PIM execution.  
While the trends for traffic and performance still remain the same for our updated results, NC now performs slightly \emph{better} than fine-grained coherence (FG) on average.  We updated our evaluation in the paper accordingly.


\end{enumerate}

\vspace{10pt}
\changesII{We have also made minor changes to improve the writing and clarity of the 
paper.}
We respond to each reviewer's feedback in detail on the following pages, and describe the
associated changes we made to the revised paper.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage %\vspace{20pt}
\subsection*{{\Large Reviewer 1}}

\begin{tcolorbox}[parbox=false, enhanced, frame hidden, colback=gray!50, breakable]
{\bf\large Question 1.1}

It is important to give some intuition about why some programs need concurrent access from both sides. Prior work mostly assumes coarse-grained separated access and it seems to work well for many apps. Sometimes this is even preferred as it reduces ping pong data back and forth. Even with perfect coherence protocol this is still not acceptable as the data need to be transferred back and forth. 
\end{tcolorbox}


We believe that there are two points to address in the reviewer's comments. 

First, we found that for a number of important classes of applications, both the portions executing on PIM and the portions executing on the processor access the same data structures. One class of examples are multithreaded graph processing frameworks, such as Ligra~\cite{ligra}, where multiple threads operate on the same shared in-memory graph~\cite{Seraph,ligra}. Each thread executes a graph algorithm, such as the popular PageRank. We studied a number of these algorithms~\cite{ligra} and found that when we converted each of them for PIM execution, only some portions of each algorithm were well suited for PIM, while the remaining portions performed better if they stayed on the processor. This observation was also made by prior work~\cite{Ahn:2015:PIL:2749469.2750385}.  With this partitioning, some threads execute the processor portion while other threads (sometimes concurrently) execute the PIM portion, with all of the threads sharing the graph and other intermediate data structures.

Another example is an modern in-memory database that supports hybrid transactional/analytical processing (HTAP) workloads. Today, \changesII{analytical} and transactional \changesII{operations} are being combined in a single hybrid database system, as observed in several academic and industrial databases~\cite{SAP,MemSQL,stonebraker2013voltdb}, thanks to the need to perform real-time analytics on transactional data. The \changesII{analytical} portions of these hybrid databases are well suited for PIM execution, as analytical queries have long lifetimes and touch a large number of database rows, leading to a large amount of random memory accesses and data movement~\cite{Hash:NME,JAFAR,kocberber2013meet}. On the other hand, even though transactional queries access the same data, they likely perform better if they stay on the processor, as they are short-lived and are often latency sensitive, accessing only a few rows each. In such workloads, concurrent accesses from both PIM kernels and processor threads are inevitable, as analytical queries benefit from executing near the data while transactions perform best \changesII{when executed on the} processor cores.

Second, we believe that providing a highly efficient and lightweight coherence mechanism in hardware, like LazyPIM, can enable new applications that perform fine-grained sharing between processor cores and PIM cores. In other words, LazyPIM can potentially be an enabling mechanism for applications we cannot envision today. We believe this is similar to applications that make use of both the processor and the GPU. Enabling fine-grained coherence across such accelerators can lead to new applications taking advantage of such mechanisms. 


%\newpage %
\vspace{15pt}
\textbf{We modified the beginning of Section 3, as follows, to address the \changes{reviewer's comments:}}
\vspace{-5pt}
\begin{tcolorbox}[enhanced, frame hidden, colback=yellow!50, breakable, before upper={\parindent14pt}]
Prior work mostly assumes that there is only a limited
amount of sharing between the PIM kernels and the processor.
However, this is not the case for many important applications,
such as graph and database workloads. For example, in multithreaded
graph frameworks, each thread performs a graph
algorithm (e.g., connected components, PageRank) on a shared
graph~[26, 31]. We study a number of these algorithms~[26],
and find that (1)~only certain portions of each algorithm are
well suited for PIM, and (2)~the PIM kernels and processor
threads access the shared graph and intermediate data structures
concurrently. Another example is modern in-memory
databases that support Hybrid Transactional/Analytical Processing
(HTAP) workloads~[18, 22, 29]. The analytical portions of
these databases are well suited for PIM execution~[15, 19, 30].
On the other hand, even though transactional queries access the
same data, they perform better if they stay on the processor, as
they are short-lived and latency sensitive, accessing only a few
rows each. Thus, concurrent accesses from both PIM kernels
(analytics) and processor threads (transactions) are inevitable.

As a result of sharing, the data need to remain coherent
between the processor and PIM cores...
\end{tcolorbox}



\vspace{30pt}
\begin{tcolorbox}[parbox=false, enhanced, frame hidden, colback=gray!50, breakable]
{\bf\large Question 1.2}

What applications require the fine-grained coherence support? Is fine-grained coherence support really helpful?
\end{tcolorbox}  


First, fine-grained coherence is very important for applications that use pointer-intensive data structures, such as graph workloads and databases. The path taken while traversing the pointers is not known ahead of time.  As a result, even though a thread often accesses only a few dispersed pieces of the data structure, a coarse-grained mechanism has no choice but to acquire coherence permissions for the \emph{entire} data structure. When a PIM kernel acquires coherence on the data structure, if a processor thread wants to access any part of that data structure, the coarse-grained mechanism either generates a lot of ping-ponging of coherence permissions between the processor and PIM, or forces one side (i.e., either the processor or the PIM) to stall when the other side has permissions, greatly hurting the performance benefits attainable by PIM execution.  Fine-grained coherence avoids this by acquiring permissions on only the pieces of data within the shared structure that are actually accessed by the processor or PIM cores. We found that coarse-grained approaches were too conservative \changes{for our applications}, as the individual pieces of data (i.e., the cache lines) accessed by the processor and by the PIM cores \changesII{often did not} overlap (thus avoiding the need for most ping-ponging). This is supported by the analysis and data we provided in the submission. 

Second, fine-grained coherence can ease programmer effort in partitioning data between PIM cores and the processor. Prior works on PIM that use coarse-grained coherence either eliminate a significant portion of the potential PIM benefits (as we discuss above and show in our results) or force programmers to perform significant code transformations to minimize ping-ponging. We proposed LazyPIM as a way of enabling the performance benefits of PIM through efficient fine-grained coherence support, without requiring significant changes to the programming approach.  Note that to use coarse-grained mechanisms, programmers often have to perform more significant code transformations.  \changes{Nothing prevents programmers from executing such refactored code on LazyPIM.} 
%- in fact, they will still see most of the benefits that they would have with coarse-grained mechanism.

Finally, as we mentioned in our response to Question 1.1, we believe that enabling fine-grained coherence \changesII{between processor cores and accelerators, such as PIM cores,} can lead to new applications taking advantage of such mechanisms.


\vspace{15pt}
\textbf{We modified Section 3, as follows, to address the reviewer's comments:}
\vspace{-5pt}
\begin{tcolorbox}[enhanced, frame hidden, colback=yellow!50, breakable, before upper={\parindent14pt}]
As a result of sharing, the data need to remain coherent
between the processor and PIM cores. Traditional, or \emph{fine-grained},
coherence protocols (e.g., MESI) have several qualities
well suited for pointer-intensive data structures, such as those
in graph workloads and databases. Fine-grained coherence allows
the processor or PIM to acquire permissions for only the pieces
of data that are actually accessed. In addition, fine-grained
coherence can ease programmer effort when developing PIM
applications, as multithreaded programs already use this
programming model.
\end{tcolorbox}



\vspace{35pt}
\begin{tcolorbox}[parbox=false, enhanced, frame hidden, colback=gray!50, breakable]
{\bf\large Question 1.3}

As well known, PIM works for memory-intensive applications. These apps usually have large memory footprint, so the number of PIM core accessed addresses is large. The authors use L1 cache as the tracking table for speculative access addresses and rollback if exceeded. This may not be adequate considering the many accesses. Also, it could require too many bloom filters to track the read/write sets.
\end{tcolorbox}  


In LazyPIM, the L1 cache in the PIM cores is used to hold only data updates from speculative writes.  The \changes{addresses of speculative reads and writes are tracked} using the Bloom filter signatures (the PIMReadSet/PIMWriteSet, which are separate from the L1 cache). Speculative read \changes{addresses} are recorded \changesII{into a Bloom filter signature (the PIMReadSet)} as soon as the PIM cores issue the read, and correctness is not affected if a read gets evicted from the cache, as the signature still contains the read's address for use in conflict detection. For speculative writes, we both record the write address into \changesII{a Bloom filter signature} (the PIMWriteSet), and stage the data update in the L1 cache.

For the applications we studied, when we selected the PIM kernels, we did not take PIM L1 capacity or Bloom filter capacity into consideration.  Even then, our analysis shows that the speculative writes generated by a PIM kernel never exceeded the L1 cache capacity (and were never evicted), and that the number of reads and writes never exceeded the maximum \changes{number of addresses that our Bloom filters could hold}.

Naturally, one can expect that there could be PIM kernels that generate a lot of reads and/or writes, and exceed the L1 and/or Bloom filter capacity.  We can simply avoid this by dividing the PIM kernel into smaller chunks, where we perform a commit after each chunk completes.  This lowers the number of speculative updates and the number of addresses that must be tracked by our signatures.  In fact, this same optimization allows us to lower the Bloom filter overhead and further reduce the number of rollbacks that are triggered.  As part of our future work, we will incorporate a runtime mechanism to efficiently determine the optimal chunk size for performing commit.  For now, we simply had LazyPIM trigger a PIM core rollback whenever a PIM L1 cache needed to write back a speculative update (which squashed the writeback) or whenever the Bloom filter reached its maximum capacity (neither of which occurred for our evaluated applications).  As we described in Section 4.2.3, we included a failsafe mechanism that guarantees forward progress after 3 consecutive rollbacks.


\vspace{35pt}
\begin{tcolorbox}[parbox=false, enhanced, frame hidden, colback=gray!50, breakable]
{\bf\large Question 1.4}

The authors manually mark and offload the PIM portion of the programs. This is a non-trivial work. If not done correctly, the PIM version will have little speedup and too much unnecessary off-chip traffic. It will be good to mention the performance of the baseline w.r.t. the non-PIM version, to show that it is not a crappy baseline and the proposed solution reduces the truly necessary off-chip traffic. 
\end{tcolorbox}


We updated our results to include the performance of the non-PIM (i.e., \emph{CPU-only}) \changesII{system}.  This data is now included in Figures~1 and~4 in the paper, as shown below.  To illustrate the impact of off-chip traffic and inefficient coherence mechanisms, we also showed the performance of a theoretical ideal PIM mechanism (\emph{Ideal-PIM}), where we can perform fine-grained \changesII{coherence} for free (i.e., there is no latency or bandwidth associated with a coherence request).  We make three conclusions from this data.  First, without any coherence overhead, the ideal PIM mechanism significantly outperforms the CPU-only \changesII{system} for all of our applications.  Second, a good PIM coherence mechanism is essential for PIM performance.  For example, fine-grained coherence (\emph{FG}) and coarse-grained locks (\emph{CG}) \changesII{often} lead to a \emph{performance loss} over a baseline without PIM (Figure~4, right), and for 16-thread PageRank running on the Gnutella graph, all prior mechanisms \changes{lead to performance loss over CPU-only} (Figure~4, right). Third, LazyPIM, with its efficient approach to fine-grained coherence, can achieve performance results very close to Ideal-PIM.

\vspace{15pt}
\textbf{We replaced Figure~1 in Section~3, as follows, to address the reviewer's comments:}
\vspace{-5pt}
\begin{figure}[h]
\vspace{-5pt}
\begin{tcolorbox}[enhanced, frame hidden, colback=yellow!50, breakable, before upper={\parindent14pt}]
\noindent
... Fig. 1 shows the speedup of different
coherence mechanisms for certain graph workloads, normalized
to a CPU-only baseline (where the entire application runs
on the processor cores). To illustrate the impact of inefficient
coherence mechanisms, we also show the performance of an
ideal PIM mechanism where there is no performance penalty
for coherence (Ideal-PIM). As shown in Fig. 1, fine-grained
coherence (FG) never performs better than CPU-only.\\

\begin{minipage}[t]{0.95\linewidth}
\centering
\begin{minipage}[t]{0.7\textwidth}
    % \vspace{-3pt}
    \centering
    \includegraphics[width=\linewidth]{figures/Motivation-1.pdf}
\end{minipage}
    \caption*{Fig.~1. Speedup for Facebook and Gnutella graph with 16 threads, normalized to CPU-only.}
\end{minipage}
\end{tcolorbox}
\end{figure}

\vspace{20pt}
\textbf{We modified Figure~4 in Section~6, as follows, to address the reviewer's comments:}
\vspace{-5pt}
\begin{tcolorbox}[enhanced, frame hidden, colback=yellow!50, breakable, before upper={\parindent14pt}]
Fig. 4 (left) shows the performance of PageRank using
Gnutella as we increase the thread count. LazyPIM comes
within 6.0\% of Ideal-PIM (as defined in Sec. 3), and improves
performance by 73.2\% over FG, 47\% over CG, 29.4\% over NC,
and 39.4\% over CPU-only on average. With NC, the processor
threads incur a large penalty from going to DRAM frequently.
CG suffers greatly due to (1) flushing dirty cache lines, and
(2) blocking all processor threads that access PIM data during
execution. In fact, processor threads are blocked for up to 73\%
of the total execution time with CG. With more threads, the
effects of blocking worsen CG’s performance. FG also loses a
significant portion of Ideal-PIM’s improvements, as it sends a
large amount of off-chip messages.

Fig. 4 (right) shows the performance improvement for
16 threads. Without any coherence overhead, Ideal-PIM significantly
outperforms CPU-only across all applications, showing
the affinity of the applications to PIM. Poor handling of coherence
by FG, CG, and NC leads to dramatic performance losses
compared to Ideal-PIM, indicating that an efficient coherence
mechanism is essential for PIM performance. For example, in
some cases, NC and CG actually performs worse than CPUonly,
and for PageRank running on the Gnutella graph, all
prior mechanisms have performance loss. In contrast, LazyPIM
consistently retains most of Ideal-PIM’s benefits for all applications,
coming within 5.5\% on average. LazyPIM also outperforms
all of the other approaches, even though 38.5\% of its
kernels roll back due to concurrent accesses from the processor.
\end{tcolorbox}

%\newpage
\vspace{-10pt}
\begin{figure}[h]
\vspace{-5pt}
\begin{tcolorbox}[enhanced, frame hidden, colback=yellow!50, breakable, before upper={\parindent14pt}]
\centering
\begin{minipage}[t]{0.7\textwidth}
    % \vspace{-3pt}
    \centering
    \begin{minipage}{0.354\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/performance1.pdf}
    \end{minipage}%
    \hfill%
    \begin{minipage}{0.646\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/performance2.pdf}
    \end{minipage}%
\end{minipage}
    \caption*{Fig.~4. Speedup sensitivity to thread count for PageRank with Facebook graph (left), and speedup for all applications with 16~threads (right) for coherence mechanisms, normalized to CPU-only.}
\end{tcolorbox}
\end{figure}



\newpage %\vspace{15pt}
\begin{tcolorbox}[parbox=false, enhanced, frame hidden, colback=gray!50, breakable]
{\bf\large Question 1.5}

Also, the best way to separate programs for coarse and fine grained coherence may be different. It is important to compare the best of each, not a good one for one and a bad one for the other.
\end{tcolorbox} 


\changes{Yes --- we compared using the best partitioning we could find for each coherence mechanism, but we found that \emph{for our applications}, the best for each was in fact the same across all PIM coherence mechanisms.  This is because for each of these mechanisms, the best partitioning is likely one that minimizes the amount of data shared between the processor cores and PIM cores.}

Our goals during partitioning were to lower execution time and minimize data movement, which all PIM mechanisms aim to achieve~\cite{Ahn:2015:PIL:2749469.2750385,Mingyu:PACT,7056040}.  As prior work~\cite{Ahn:2015:PIL:2749469.2750385} has shown, parts of the application that are either (1)~compute-intensive or (2)~cache-friendly should remain on the processor, as they can benefit from larger, more sophisticated cores with larger caches (as opposed to the small PIM cores).  Thus, only memory-intensive portions of the code with poor cache locality were dispatched to the PIM cores for execution.  To partition an application, we profiled its execution time, along with its miss rate over each function.  Based on the profiling information, we selected candidate PIM portions conservatively, choosing portions where (1)~the application spent a majority of its cycles (to amortize the overhead of launching PIM execution), and (2)~a majority of the total last-level cache misses occurred (indicating high memory intensity and poor cache locality).  \changes{From this set of candidate kernels, we selected only the kernels \emph{for each mechanism} that had minimal coherence overhead \changesII{for that particular} mechanism (i.e., they minimized the communication that occurred between the processor threads and the PIM kernels).}

\changes{
For the applications that we studied, due to the structure of their underlying algorithms, the kernels chosen for each PIM coherence mechanism ended up being the same, \emph{despite the different target partitioning goals of each mechanism}.  Ultimately, we found that \emph{all of the PIM coherence mechanisms benefited the most when we minimized the amount of data sharing} between the processor and PIM cores, hence why the kernels chosen were identical. \changesII{(We describe why in detail below, under \emph{More Detail on Best Partitioning for Prior PIM Mechanisms}.)}  Ideally, we wanted to eliminate sharing completely, but due to the inherent design of our applications, this could be reasonably achieved only by executing the entire application on the PIM cores.  As Figure~\ref{fig:nopim} shows, this approach (\emph{PIM-only}) can hurt performance significantly, as the PIM cores are weaker than processor cores and have smaller caches, slowing down parts of the application that were better suited for processor execution.  Therefore, to keep these parts on the processor, some minimal data sharing was unavoidable for our applications.  When we partitioned our applications in this way, we saw that they showed significant performance benefits over the unmodified code (\emph{CPU-only}) if we used an ideal PIM coherence mechanism (\emph{Ideal-PIM}) with no coherence overheads (also shown in Figure~4 in the paper for all of our applications).
}

\begin{figure}[h]
\vspace{-5pt}
%    \centering
    %\begin{minipage}{1\linewidth}
        \centering
        \includegraphics[scale=0.5]{figures/nopim.pdf}
    %\end{minipage}%
    \captionsetup{justification=centering}
  %  \rule{1cm}{1cm}
    \caption{Speedup for Radii and Connected Components with 16 threads if applications run only on PIM cores or with an ideal PIM mechanism (where there is no coherence overhead), normalized to CPU-only.}
    \label{fig:nopim}
\end{figure}

%\changes{
%To evaluate the effectiveness of our partitioning approach, we executed the partitioned applications using an ideal PIM coherence mechanism with no coherence overheads (\emph{Ideal-PIM} in Figure~\ref{fig:nopim}). With the ideal mechanism, our partitioning resulted in significant performance benefits over the unmodified code (CPU-only), which was corroborated across all of our applications (Figure~4 in the paper).  These kernels achieved high speedups under Ideal-PIM because they limited the actual amount of data sharing that occurred between the processor cores and PIM cores, while still (1)~reducing data movement between DRAM and the processor, and (2)~not migrating code that is best-suited for processor core execution to the PIM cores.  Unfortunately, while the kernels that we selected were amenable to PIM, the overheads of prior PIM coherence mechanisms remained very high and undid most of the performance benefits, as these mechanisms were not inherently a good fit for applications such as ours.}

Note that while we did our best to select what we believe are PIM portions that achieve near-maximum performance for our applications on prior PIM mechanisms, there may be other approaches that find the \emph{most optimal} partitioning. However, we believe such approaches are outside the scope of this paper.

% When we partition programs into PIM portions and CPU portions, our goal is to lower execution time and minimize data movement, which are goals that all PIM mechanisms aim to achieve \cite{Ahn:2015:PIL:2749469.2750385,Mingyu:PACT,7056040}.  As prior work \cite{Ahn:2015:PIL:2749469.2750385} has shown, parts of the application that are either (1) compute-intensive or (2) cache-friendly should remain on the CPU, as they can benefit from larger, more sophisticated cores with larger caches (as opposed to the small PIM cores).  Thus, memory-intensive portions of the code with poor cache locality are dispatched to the PIM cores for execution.  To partition an application, we profile its execution time, along with its miss rate over each function.  Based on the profiling information, we select the PIM portions conservatively, choosing a single portion where (1) the application spends the majority of its cycles (to amortize the overhead of launching PIM execution), and (2) the majority of last-level cache misses occur (indicating high memory intensity and poor cache locality).  As Figure~4 shows below, we find that our PIM kernel selection can result in significant performance benefits over the unmodified code (i.e., CPU-only execution) if we assume no coherence overhead when communicating between PIM kernels and CPU cores (i.e., Ideal-PIM).

% Naturally, all practical mechanisms for PIM coherence incur some form of communication overhead, whenever data is shared between the PIM portion and the CPU portion. In an ideal world, we would eliminate sharing completely. However, for our applications, without completely rewriting them, the only way to get rid of sharing is to execute the entire program on the PIM cores. Such an approach hurts significantly, as we show for Radii and Connected Components in Figure~\ref{fig:nopim} (shown as \emph{PIM-only}). This occurs because the PIM cores are weaker than the CPU cores and have much smaller caches, due to limitations on the complexity and size of the logic that can be integrated within memory. Therefore, moving portions of the code that are compute-intensive or that benefit from large caches can be highly detrimental to performance.


% In trying to ensure that the portions of an application that benefit the most from CPU execution are not dispatched to PIM cores, there can be cases where despite our best efforts to eliminate data sharing, some sharing must inevitably occur between the CPU threads and PIM kernels.  We choose PIM/CPU partition boundaries such that they minimize the amount of data sharing that occurs between the PIM portions of the application and the CPU portions. To understand why this is beneficial for all PIM coherence mechanisms, we briefly analyze what happens to each of them when sharing occurs. In all of these mechanisms, when the PIM kernel is not running, the overhead of coherence is minor. As a result, we examine the overheads that occur when the PIM kernel is running, and the CPU wants to share data (i.e., the CPU accesses PIM data during PIM kernel execution).


\vspace{10pt}
\changes{\underline{\bf\em \changesII{More Detail on} Best Partitioning for Prior PIM Coherence Mechanisms}}

\changesII{In this section, we describe in detail how we chose PIM kernels independently for each PIM coherence mechanism, and why despite this independent selection process the same kernels ended up being chosen by all mechanisms for our applications.}

\vspace{5pt}
{\bf Coarse-Grained Mechanisms.}
\changes{
Coarse-grained PIM coherence mechanisms experience high coherence overhead whenever the processor tries to access PIM data while the PIM kernel holds the coherence permissions for this data.  Depending on the mechanism, this overhead can be one of three costs: (1)~processor execution blocks until the PIM kernel completes; (2)~the requested data ping-pongs between the processor and the PIM cores; or (3)~to avoid conflicts during PIM execution, a greater number of cache lines need to be preemptively flushed by the processor.  Prior work was able to minimize these overheads \emph{for the applications they selected}, as their processor threads and PIM kernels either worked on independent sets of data or shared very little of the data concurrently~\cite{Mingyu:PACT,7056040,JAFAR}.  Many other applications, including ours, commonly have access \changesII{patterns, such as pointer chasing, running} on multiple threads, where it is hard to predict the pieces of data the threads will access, and therefore hard to partition them to work on independent sets.} As a result, the best way to minimize the coherence overhead for these applications is to \emph{minimize the amount of data sharing that occurs between PIM cores and the processor}. Prior work on coarse-grained PIM coherence has corroborated this, stating that an ideal application requires only infrequent sharing and communication at well-defined points throughout the application~\cite{Mingyu:PACT}.
%Coarse-grained PIM coherence mechanisms either maintain a single coherence entry or lock part or all of the PIM data. During PIM execution, the PIM kernel will hold the lock on PIM data.  An access during this time from the CPU to PIM data can result in significant performance penalties, by (1)~blocking CPU execution until the PIM kernel completes; (2)~causing the requested data to ping-pong between the CPU cores and PIM cores; or (3)~requiring a greater number of cache lines to be flushed before PIM execution starts, in order to avoid conflicts during PIM execution.  If the access pattern is predictable, such behavior can be reduced by shrinking the size of the data that is locked by PIM.  However, for many applications such as ours, common access patterns such as pointer chasing are very difficult to predict ahead of time, thus making it impractical to shrink the size of locked data significantly.  As a result, the best way to minimize the coherence mechanism overhead is to \emph{minimize the amount of data sharing that occurs between PIM cores and CPU cores}. Prior work on coarse-grained PIM coherence has corroborated this, stating that an ideal application requires only infrequent sharing and communication at well-defined points throughout the application~\cite{Mingyu:PACT}.

\vspace{5pt}
{\bf Non-Cacheable Mechanisms.}
\changes{
For non-cacheable mechanisms, all processor requests to PIM data cannot be cached, and must go off-chip.  \changesII{In applications well suited for PIM,} a major reason that some portions of code benefit from executing on the processor is high cache locality, which can take advantage of the large caches on the processor.  By preventing caching for shared PIM data, non-cacheable mechanisms undo this benefit, instead incurring a large overhead every time the processor makes a request to this data. To avoid this overhead, prior work simply migrated all parts of the code that access PIM data to the PIM cores~\cite{Ahn:2015:SPA:2749469.2750386}. For the applications we studied, due to their underlying algorithms, this requires us to port the entire application to the PIM cores, which as we saw in Fig.~\ref{fig:nopim} performs poorly.  As a result, to minimize the performance degradation, we want to minimize the number of requests that are forced to go off-chip (i.e., the number of processor requests to shared data) while still keeping code that is compute-intensive or has high cache locality on the processor.  Effectively, this means that we want to partition our code such that we \emph{minimize the amount of data sharing that occurs between PIM cores and the processor}.
}
%For non-cacheable mechanisms, all processor requests to PIM data go off-chip.  While this doesn't require coherence to be performed on PIM data, the processor portion of the code, which benefits from having a large cache, can no longer utilize the cache.  When the processor makes many requests to the shared data, this loss of cache utilization results in performance similar to executing the entire application on the PIM cores.  As a result, we want to minimize the performance degradation, which can be done by minimizing the number of requests that are forced to go off-chip (i.e., the number of processor requests to shared data).  \changes{We can achieve this by \emph{minimizing the amount of data sharing that occurs between PIM cores and the processor}.}

\vspace{5pt}
{\bf Fine-Grained Mechanisms.}
When we perform fine-grained coherence in a system such as ours, where we have hierarchical coherence using two directories (the processor directory and the PIM directory), coherence overheads occur when messages must be sent across the two directories (i.e., if the coherence status does not exist in the local directory).  \changes{Such coherence misses occur more frequently when the data moves frequently between the processor and the PIM cores, as the coherence permissions for the data keeps moving between the processor directory and the PIM directory.  We can minimize the number of coherence misses that occur by maximizing the probability that a piece of data being accessed remains in the local caches (and therefore in the local directory).  To achieve this, \emph{the amount of data sharing between the PIM cores and processor should be minimized}.}
%These overheads occur only when the CPU portion of the program requests data in the PIM cache, and the PIM portion of the program requests data in the CPU cache (i.e., when data is being shared between the two portions of the program).  To minimize the overhead, we must minimize the number of messages sent across the two directories, by minimizing the amount of data shared between the two.

\vspace{5pt}
As we can see, the differences between the coherence mechanisms are exposed whenever sharing occurs, which in all cases incurs a performance overhead.  Thus, by minimizing sharing, our partitioning methodology picked PIM kernels \changes{for our applications} that were a good fit for \emph{all} of the coherence mechanisms.  Note that LazyPIM attains performance improvements over prior coherence mechanisms whenever sharing occurs.  As the goal of our methodology is to minimize the number of times that sharing occurs, we do not exaggerate (and maybe even downplay) the benefits that LazyPIM has over prior mechanisms in our results --- 
%a different selection methodology would greatly hurt the prior mechanisms' performance
\changesII{a different selection methodology that increases the amount of data sharing would be detrimental to prior mechanisms, greatly hurting the mechanisms' performance and thus potentially providing greater margins of improvement for LazyPIM.} \changes{Again, while we did our best to select a near-optimal partitioning for these prior PIM coherence mechanisms, there may be other approaches that find the \emph{most optimal} partitioning, but we believe such approaches are outside the scope of this paper.}


\vspace{15pt}
\textbf{We modified Section~5, as follows, to address the reviewer's comments:}
\vspace{-5pt}
\begin{tcolorbox}[enhanced, frame hidden, colback=yellow!50, breakable, before upper={\parindent14pt}]
PIM kernels are selected from these applications with the help of OProfile~[20].
We conservatively select candidate PIM kernels, choosing hotspots
where the application (1)~spends the majority of its
cycles, and (2)~generates the majority of its LLC misses.
From these candidates, we pick kernels that we believe minimize 
the coherence overhead for each evaluated mechanism, by minimizing
data sharing between the processor and PIM cores.
We modify each application to ship the hotspots to
the PIM cores.  We manually annotate the PIM data set.
\end{tcolorbox}



\vspace{35pt}
\begin{tcolorbox}[parbox=false, enhanced, frame hidden, colback=gray!50, breakable]
{\bf\large Question 1.6}

How large the PIM kernels should be? If PIM kernels are small but commit takes long time, the PIM benefits can be offset. If the PIM kernels are too large, then there might be too many rollbacks. How could the programmer or compiler decide an optimal kernel size? 
\end{tcolorbox}


For small PIM kernels, the overhead of initializing the kernel can often outweigh the benefits of execution.  For this paper, we only \changes{picked hotspots} from each application, where the majority of total execution cycles for the application were spent according to OProfile~\cite{oprofile}.  As our results \changesII{show}, the performance improvement of LazyPIM due to accelerating these hotspots outweighs the overheads of initialization.  As we mentioned in our answer to Question 1.3, there is no rule that prohibits \changesII{the use of} a PIM kernel of a large size.  \changes{We found that} \changesII{even when an application had a majority of its kernels roll back at least once,}
%rollbacks occurred 38.7\% of the time, on average, for the kernels that we selected, and even with that many rollbacks,} 
we were still able to attain significant performance improvements with LazyPIM.

Picking the optimal size of kernels is a different problem from what we are trying to solve in this work. We believe there is a lot of opportunity for future work in this area, but we believe it is beyond the scope of our work.\\



\newpage %\vspace{30pt}
\begin{tcolorbox}[parbox=false, enhanced, frame hidden, colback=gray!50, breakable]
{\bf\large Question 1.7}

According to 4.2.3, commit requires significant invalidations on processor side (thus future cache misses) and writebacks on PIM side. Will this be a large overhead for small PIM kernels? Has your evaluation consider this?
\end{tcolorbox}


\changes{Yes ---} our evaluation considered the full overhead of a commit, including the latency of sending the signatures from the PIM core to the processor (40~cycles per signature), the latency of comparing all of the processor signatures against the PIM core signatures (2~processor cycles per comparison, which is more conservative than assumed by prior work~\cite{bulksc}), and the latency of performing processor-side cache invalidations on any matching (i.e., conflicting) addresses (8~cycles for an invalidation in the tag store).  As prior work has shown~\cite{bulksc}, detecting conflicts by calculating the intersection of two Bloom filters is a low-cost operation that can be done using simple bitwise logic.  Note that during commit, no writebacks occur on the PIM side, as we simply clear the speculative bits in the PIM cache and have subsequent accesses from the CPU to DRAM query the PIM coherence directory. 

We found that the overhead of commit for our applications is negligible.  With 16 cores, the average commit overhead for our applications was 0.78\% of total execution time.  The overhead was low because (1)~the processor threads did not stall during this invalidation phase unless they accessed PIM data, reducing the impact of the overhead on the critical path of latency; and (2)~the PIMWriteSet typically contained only a small number of addresses (1532 on average). For smaller PIM kernels, this overhead was lower, as the signatures contains fewer addresses (requiring fewer conflict checks and fewer processor cache invalidations); therefore, the size of the PIM kernel is directly correlated with the length/overhead of commit.



\newpage %\vspace{20pt}
\subsection*{{\Large Reviewer 2}}

\begin{tcolorbox}[parbox=false, enhanced, frame hidden, colback=gray!50, breakable]
{\bf\large Question 2.1}

The conflict between Processor-write and PIMcore-read are detected and resolved, but the Processor-write and PIMcore-write (RAW) dependencies are not clearly described. I think all the data dependencies scenarios should be discussed.
\end{tcolorbox}


As we discussed in Section 4, we used coarse-grained atomicity in LazyPIM, where all of a PIM kernel's memory operations effectively take place at commit time, and all PIM memory operations that occur during PIM kernel execution are speculative (i.e., are not committed to system state) until commit is reached. This means that any memory instructions that are part of a PIM kernel can be thought of as being batched together into a single operation issued at commit time, and that all processor memory instructions that take place during PIM kernel execution are ordered before the PIM kernel's memory operations. We now discuss the possible interleavings for operations from both the processor and PIM to the same cache line, assuming a sequential consistency memory model (though \changes{this argument} can easily be applied to other memory consistency models, such as x86-TSO).

\vspace{5pt}
{\bf PIM Read and Processor Write to the Same Cache Line.}
\emph{This is a conflict.} Any PIM read during the kernel execution should be ordered after the processor write (RAW, or read-after-write). However, because the PIM core does not check coherence throughout execution, the PIM read operation reads potentially stale data from DRAM instead of the output of the processor write (which sits in the processor cache). This is detected by the LazyPIM mechanism, resulting in rollback and re-execution of the PIM kernel after the processor write is flushed to DRAM.

\vspace{5pt}
{\bf Processor Read and PIM Write to the Same Cache Line.}
\emph{This is not a conflict.} With coarse-grained atomicity, any read by the processor during PIM execution is ordered before the PIM core's write (WAR, or write-after-read). As a result, the processor should not read the value written by PIM.  LazyPIM ensures this by marking the PIM write as speculative and maintaining \changes{the speculative data} in the PIM cache, preventing processor read requests from seeing any data flagged as speculative.

Note that if the programmer wants the processor's read to see the PIM core's write, they would have to use a synchronization primitive (e.g., memory barrier) to enforce ordering between the processor and the PIM core. This scenario is identical to a conventional multithreading environment, in which the explicit ordering of memory operations must be enforced by the programmer using synchronization primitives, which are supported by LazyPIM.

\vspace{5pt}
{\bf Processor Write and PIM Write to the Same Cache Line.}
\emph{This is not a conflict,} as either ordering of the write is valid in the consistency model.  With coarse-grained atomicity, the processor's write is ordered before the PIM core's write (WAW, or write-after-write). As with any conventional multithreaded application, if the programmer wishes to enforce a specific ordering of the two writes, they must insert synchronization primitives, such as a write fence.


\vspace{15pt}
\textbf{We modified Section~4.1, as follows, to address the reviewer's comments:}
\vspace{-5pt}
\begin{tcolorbox}[enhanced, frame hidden, colback=yellow!50, breakable, before upper={\parindent14pt}]
If the PIM kernel writes to a cache line that is subsequently
read by the processor before the kernel finishes (e.g., the second
write by PIM0 to line B in Fig. 2), this is not a conflict. With
coarse-grained atomicity, any read by the processor during PIM
execution is ordered before the PIM kernel's write. LazyPIM ensures
that the processor cannot read the kernel's writes, by marking
them as speculative until the kernel finishes (see Sec. 4.2.2). This
is also the case when the processor and a PIM kernel
write to the same cache line. Note that this ordering does not
violate consistency models\changes{,} such as sequential consistency.
\end{tcolorbox}



\vspace{30pt}
\begin{tcolorbox}[parbox=false, enhanced, frame hidden, colback=gray!50, breakable]
{\bf\large Question 2.2}

The example in Fig.2, A and C are both written by CPU0. In section 4.1, it is described that CPU1 writes to line A, the description and the figure should be consistent.
\end{tcolorbox}


We fixed the text in Section 4.1 to match Figure 2. 


\vspace{5pt}
\textbf{We modified Section 4.1, as follows, to address the reviewer's comments:}
\vspace{-5pt}
\begin{tcolorbox}[enhanced, frame hidden, colback=yellow!50, breakable, before upper={\parindent14pt}]
\noindent ... Fig.~2 (left) shows two examples of this: (1)~CPU0's write to line~C during kernel execution; and (2)~CPU0's write to line~A \emph{before} kernel execution, which was not written back to DRAM...
\end{tcolorbox}



\newpage %\vspace{15pt}
\begin{tcolorbox}[parbox=false, enhanced, frame hidden, colback=gray!50, breakable]
{\bf\large Question 2.3}

if energy effect can be evaluated and included will be more comprehensive.
\end{tcolorbox}


Unfortunately, our current infrastructure cannot provide us with reliable energy numbers for the PIM cores.  We plan to extend the infrastructure to accurately model this in the future.  Given the simplicity of the PIM cores, along with the significant reduction in execution time \changes{and memory bandwidth} over CPU-only execution (see Figures~3 and~4 in the paper), we expect to see some reductions in total energy consumption, but we do not have quantitative data to \changesII{show} this at the moment.



\vspace{30pt}
\begin{tcolorbox}[parbox=false, enhanced, frame hidden, colback=gray!50, breakable]
{\bf\large Question 2.4}

In section 4.2.3, conflicts are detected between CPUWriteSet and PIMReadSet, is it guaranteed that CPU will not read the stale data written by the PIM kernel? How to guarantee that? (Section 4.1 mentioned it's not a conflict, what if the processor depends on the  PIMcore write and need to read the updated value? Does it wait until the kernel finishes due to non-speculation, is that will affect the correctness as well as degrade the performance?)
\end{tcolorbox}


We ensured that the processor can never read stale data written by the PIM kernel.  Due to the coarse-grained atomicity used for PIM kernel memory accesses, PIM kernel writes do not effectively take place until commit takes places.  To ensure this coarse-grained atomicity, we flagged all uncommitted PIM writes as speculative. When any processor read request misses in the on-chip last-level cache, it goes to main memory, and is unable to read data flagged as speculative from the PIM caches. Note that we do not violate consistency models by enforcing this ordering\changes{, as we described in our response to Question 2.1.}

If the programmer explicitly wishes for a processor thread to read the value written by PIM, a synchronization primitive, such as a fence/barrier, is required to enforce the dependency. Because a PIM kernel's writes become visible at the point where the PIM kernel ends (i.e., when it commits), the barrier dependency will force the processor thread to wait until PIM kernel execution has completed. \changes{If the programmer chooses to add many other instructions into the same PIM kernel that follow the write being synchronized, there will be a performance penalty, but the correctness of the execution will not be affected.}
%While this may incur a performance penalty if the programmer chooses to allow many other instructions to follow the dependent write as part of the same PIM kernel, correctness of the execution will not be affected.


%\newpage %
\vspace{15pt}
\textbf{We modified Section~4.1, as follows, to address the reviewer's comments:}
\vspace{-5pt}
\begin{tcolorbox}[enhanced, frame hidden, colback=yellow!50, breakable, before upper={\parindent14pt}]
\noindent ... LazyPIM ensures
that the processor cannot read the kernel's writes, by marking
them as speculative until the kernel finishes (see Sec. 4.2.2). This
is also the case when the processor and a PIM kernel
write to the same cache line. Note that this ordering does not
violate consistency models, such as sequential consistency.
\end{tcolorbox}



\vspace{30pt}
\begin{tcolorbox}[parbox=false, enhanced, frame hidden, colback=gray!50, breakable]
{\bf\large Question 2.5}

It seems the PIM cache should be able to hold the working set for the PIM kernel, otherwise, the speculation and conflict detection are pure overheads?
\end{tcolorbox}


Please see our answer to \textbf{Question 1.3}.  




%\newpage%
\newpage %\vspace{20pt}
\subsection*{{\Large Reviewer 3}}

\begin{tcolorbox}[parbox=false, enhanced, frame hidden, colback=gray!50, breakable]
{\bf\large Question 3.1}

Most of all, IMHO the performance comparison is unfair.
To use PIM, applications should be partitioned into CPU-portion and PIM-portion. Like accelerators, partitioning applications for PIM should be done carefully considering the benefits of CPU/PIM and the overhead of communication.
When coherence is supported in PIM, the trade-off between PIM and CPU becomes different from that of PIM without coherence. As a result, the partitioning (or target application) should be different for PIM with coherence and without coherence.
It is not mentioned in this paper, but it seems that the same portion of code is offloaded to PIM for all methods (FG, CG, NC, and LazyPIM). If it is, then the comparison would give a wrong idea to the readers. If the authors did differently partition for each methos, it should be clearly stated with more details about the partitioning method.
\end{tcolorbox}


Please see our answer to \textbf{Question 1.5}.  We picked a methodology that was designed to maximize the performance of prior PIM coherence mechanisms, by minimizing the amount of data sharing that took places between the CPU threads and PIM kernels.  This methodology has no bias towards LazyPIM, and in fact, we believe it downplays the benefits that LazyPIM can deliver when data sharing must take place.\\



\vspace{30pt}
\begin{tcolorbox}[parbox=false, enhanced, frame hidden, colback=gray!50, breakable]
{\bf\large Question 3.2}

Also, the performance for baseline (CPU only) is not shown in the figures. It is necessary for ensuring that the tested applications are suitable for coherence-supported PIM.
\end{tcolorbox}


Please see our answer to \textbf{Question 1.4}.  We added CPU-only performance numbers to our results in Figure~4 in the paper, along with the performance of an ideal PIM mechanism with no performance penalty for coherence, to show that our applications were well suited for coherence-supported PIM.  As we see in Figure~4, there are several cases where prior coherence mechanisms actually degrade performance over a baseline without PIM.



\vspace{30pt}
\begin{tcolorbox}[parbox=false, enhanced, frame hidden, colback=gray!50, breakable]
{\bf\large Question 3.3}

Only two applications are used. However, DBx1000 does not seem to be a good example for showing the efficiency of the proposed work. It would be better if authors could add another application or replace DBx1000 with another.
\end{tcolorbox}


\changes{Thank you for your feedback.}  We replaced DBx1000 with an in-house prototype of an in-memory database (IMDB) that is capable of running both transactional and analytical queries on the same database tables, and represents modern IMDBs~\cite{SAP,MemSQL,stonebraker2013voltdb} that support Hybrid Transactional/Analytical Processing (HTAP) workloads. We included a description of this new application in Section~5.  The IMDB is capable of performing simple transactional queries (similar to TPC-C) as well as analytical queries (similar to TPC-H). Our transactional workload consists of 200K transactions, each performing reads or writes on a few randomly-chosen tuples. The analytical \changesII{workload} consists of 256 analytical queries that use the select and join operations. The IMDB uses a state-of-the-art, highly-optimized hash join kernel code~\cite{Teubner:2013:MHJ:2510649.2511320} tuned for IMDBs to service the join queries.   

Given that each transactional query is short-lived and touches only a few rows, we assigned these queries to the processor cores. On the other hand, as shown by prior work~\cite{Hash:NME,JAFAR,kocberber2013meet}, analytical queries that use \changesII{select} and join operators can benefit substantially from PIM. Thus, we used the PIM cores to perform select and join operations. We simulated a system that has 64 tables, where each table consists of 64K tuples, and each tuple has 32 fields. Tuples in tables are populated by a \changes{randomly-generated} uniformly-distributed integer.  As we show in Figure~4 (see below), the IMDB has significant benefits when run with PIM.  \changesII{An ideal PIM mechanism with no coherence overhead (\emph{Ideal-PIM}) obtains a speedup of 53.6\% over the CPU-only baseline.  LazyPIM manages to retain most of Ideal-PIM's performance improvement, with a speedup of 38.7\% over CPU-only.}
% For an ideal PIM mechanism with no coherence overheads (\emph{Ideal-PIM}), it obtains a speedup of 53.6\% over the CPU-only baseline, and with LazyPIM, we achieve a speedup of 38.7\%.




\vspace{15pt}
\textbf{We modified Section 5, as follows, to address the reviewer's comments:}
\vspace{-5pt}
\begin{tcolorbox}[enhanced, frame hidden, colback=yellow!50, breakable, before upper={\parindent14pt}]
\noindent ... We also use an in-house prototype of a modern in-memory
database (IMDB) [18,22,29] that supports HTAP workloads.
Our transactional workload consists of 200K transactions,
each randomly performing reads or writes on a few
randomly-chosen tuples. Our analytical workload consists of
256 analytical queries that use the select and join operations on
randomly-chosen tables and columns.
\end{tcolorbox}

\newpage
\textbf{We modified Figure~4 in Section~6, as follows, to address the reviewer's comments:}
\vspace{-5pt}
\begin{figure}[h]
\vspace{-5pt}
\begin{tcolorbox}[enhanced, frame hidden, colback=yellow!50, breakable, before upper={\parindent14pt}]
\centering
\begin{minipage}[t]{0.7\textwidth}
    % \vspace{-3pt}
    \centering
    \begin{minipage}{0.354\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/performance1.pdf}
    \end{minipage}%
    \hfill%
    \begin{minipage}{0.646\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/performance2.pdf}
    \end{minipage}%
    \caption*{Fig.~4. Speedup sensitivity to thread count for PageRank with Facebook graph (left), and speedup for all applications with 16~threads (right) for coherence mechanisms, normalized to CPU-only.}
\end{minipage}
\end{tcolorbox}
\end{figure}




\vspace{35pt}
\begin{tcolorbox}[parbox=false, enhanced, frame hidden, colback=gray!50, breakable]
{\bf\large Question 3.4}

How does it handle the situation where there are multiple PIM kernel requests at the same time?
There might be more complicated deadlock issues and other problems.
\end{tcolorbox}


\changes{When multiple PIM kernels run together, the kernels execute on multiple PIM cores whose L1 caches remain coherent with each other through the use of a local PIM directory, as we mentioned in Section~2.  We included hardware mechanisms to allow PIM cores to interact with each other safely, ensuring that (1)~the propagation of speculative data between PIM kernels is tracked; and (2)~if a PIM kernel rolls back, other PIM kernels that read this data also roll back.  As mentioned in Section~4.2.3, we ensured that livelock does not occur if these PIM kernels are rolled back more than 3 times, guaranteeing forward progress.}

% Multiple PIM kernels can run in parallel and simultaneously request data from memory. The PIM directory guarantees that PIM L1 caches are coherent when multiple PIM kernel are running. 
LazyPIM ensures that sharing of (potentially stale) data between multiple PIM kernels does not lead to incorrect execution. Each core maintains a per-core bit vector (the speculative read bits), indicating which of the other PIM cores it read speculative data from.  Whenever a PIM core reads speculative data written by another PIM core, it sets the corresponding speculative read bit for the core that it read from. When the core is ready to commit its kernel, it checks to see whether any speculative read bits are set. If set, the core waits to perform its conflict detection until all of the cores from which it read speculatively also complete their kernels. At commit, if \changes{there are no conflicts detected in any of the signatures from all of the PIM cores that shared data}, then the commit procedure can continue for all of these cores. If a conflict is detected in \emph{any} of the PIM cores' signatures, then \emph{all} of the cores roll back.  In essence, whenever PIM cores share speculative data with each other, their memory operations are grouped together so that they all take place atomically, behaving as a single PIM kernel.

If no speculative data exchange takes place between PIM kernels, then each PIM kernel can commit independently without having to worry about any coordination.  If two independent PIM kernels try to commit at the same time, the commit process serializes the commit requests.

We faithfully modeled all of the above interactions in our evaluation.  As we mentioned in Section 4.2.3, we ensured that no livelock issues occurred due to continuous rollbacks, as LazyPIM acquires a lock for each line in the PIMReadSet after 3 rollbacks.

\changesII{We will describe all the details of our technique in an extended version, but the 4-page limit of IEEE CAL prevents us from including all details for this submission.}



\newpage %\vspace{30pt}
\begin{tcolorbox}[parbox=false, enhanced, frame hidden, colback=gray!50, breakable]
{\bf\large Question 3.5}

The proposed method made me curious about how much are the overheads for the use of bloom filter (false positive) or the PIM restart. would it possible to provide some numbers?
\end{tcolorbox}


\changes{
\textbf{Bloom Filter Overheads.}
For each 256B \changesII{Bloom filter}, we mathematically guaranteed that the \emph{false positive rate} never exceeds 20\%, limiting each \changesII{filter} to hold a maximum of 607~addresses (as stated in Section~4.2.2).  As this work is an initial study, we assumed the worst-case, that there were \emph{always} 20\% false positives whenever we performed conflict detection.  \changesII{We computed the \emph{performance overhead of false positives} using} a simple model that translates the worst-case false positives into the greatest possible number of conflicts, flushes, and invalidations.  From this model, we found that even in the worst case, false positives led to only a 0.49\% increase in total execution time.  \changesII{As we described in Section~4.2.4, the Bloom filters currently take up a total \emph{storage overhead} of 12KB per PIM core.  We expect to reduce the storage to 784B as part of future work, by dividing a kernel into smaller chunks where each chunk's addresses fit into a single 256B Bloom filter for each of our three signatures.}
}
%The Bloom filter false positives contribute to both additional conflicts and additional flushes and invalidations. Since this work is an initial study, we have taken a conservative approach --- based on the sizings from Sections 4.2.2 and 4.2.4, our Bloom filters have a false positive rate of no greater than 20\%, and so we assume that there are always the maximum number of false positives (20\%). We have computed the overhead that the false positives incur using a simple model that assumes the worst-case number of conflicts, flushes, and invalidations. This leads to a 0.49\% increase in total execution time.

\vspace{5pt}
\textbf{PIM Restart Overheads.}
The PIM restart process involves conflict detection, flushing of conflicting data, and PIM core rollback. Conflict detection requires testing the PIM signature against the CPU signatures, which we conservatively assumed takes 2 cycles (prior work shows that it can be done in 1 cycle \changes{at a reasonable clock frequency}~\cite{bulksc,Sanchez:2007:IST:1331699.1331713}). Flushing data requires a variable amount of time, depending on the number of conflicts that occur. \changes{For our applications, the average flush overhead was 0.24\% of total execution time.} The PIM core rollback simply requires restarting execution at the checkpointed PC.

We believe there is a lot of opportunity to reduce the probability that rollbacks occur, which we leave as future work based on our submission.

%We have modified the section 4.2.4, as follows, to address the reviewer's concern.



\vspace{30pt}
\begin{tcolorbox}[parbox=false, enhanced, frame hidden, colback=gray!50, breakable]
{\bf\large Question 3.6}

How does PIM handle a PIM dataset larger than its private cache?
\end{tcolorbox}


Please see our answer to \textbf{Question 1.3}.



\vspace{30pt}
\begin{tcolorbox}[parbox=false, enhanced, frame hidden, colback=gray!50, breakable]
{\bf\large Question 3.7}

Does the coherence traffics between the PIMs incur bandwidth loss?
\end{tcolorbox}


\changes{Coherence taking place between two PIM cores does not incur any off-chip bandwidth loss, as it is performed fully within the logic layer of
DRAM.  Note that we fully modeled the impact of coherence messages between a processor core and a PIM core, which consumes part of the limited off-chip bandwidth and generates contention.}
% Coherence that takes place between PIM cores does not incur any off-chip bandwidth loss, as it is performed fully inside the DRAM.  Note that we have modeled the impact that coherence between the CPU and PIM has on off-chip bandwidth.



\vspace{30pt}
\begin{tcolorbox}[parbox=false, enhanced, frame hidden, colback=gray!50, breakable]
{\bf\large Question 3.8}

minor typo :in section 4.1, "an newer" shoudl be "a newer"
\end{tcolorbox}


We fixed this in the text.


\vspace{15pt}

